ProtoPShare: Prototype Sharing for Interpretable Image Classification and Similarity Discovery

In this paper, we introduce ProtoPShare, a self-explained method that incorporates the paradigm of prototypical parts to explain its predictions. The main novelty of the ProtoPShare is its ability to efficiently share prototypical parts between the classes thanks to our data-dependent merge-pruning. Moreover, the prototypes are more consistent and the model is more robust to image perturbations than the state of the art method ProtoPNet. We verify our findings on two datasets, the CUB-200-2011 and the Stanford Cars.

==> future_plans.tex <==
Dodac informacje o lokalizacji 

Raczej lepiej chyba byłoby robić strukturę hierarchiczną

Sprawdzić czy da się robić negatywne podejście (nie ma prototypu)

Spróbowac postawić definicję interpretowalności

sprawdzić, czy zamiast logitów i softmax nie otrzymałoby się lepszych wyników gdyby brać sigomidę z multilabel -- wtedy jesteśmy w stanie wyrwać poszczególny klasyfikator, i rozsztrzygnąć czy teo jest na przykład dany gatunek, co więcej uzyskujemy informację o tym, które gatunki są podobne (tam gdzie jest 
$\geq 1/2$) -- potencjalnie też moznaby dzieki temu łatwiej ten model uczyć -- możnaby zrobić sięc pełną 3 warstwową fully-connected o dodatnich współczynnikach, jedynie na końcu przed wejściem do sigmoidy pozwalalibyśy odejmować?

Zrobić model który się może douczać, typu zacząć od dwóch klas [jeden prototyp], i potem douczać kolejne, i patrzyć jak się modyfikuje hierarchia klas - optymalnie jakby kolejne prototypy były tworzone na coraz wyższych warstwach -- wtedy te początkowe będą najprostsze i najbardziej ogólne

można zacząć od zbudowania prototypu i funkcji w $[0,1]$ która miałaby określać
prawdopodobieństwo, tak by jakoś liczona wspólna informacja między tym wynikiem a prawdziwą klasą była maksymalna

do dyskusji: zbudowanie modelu klasyfikacyjnego na bazie rand index -- wtedy na przykład możnaby zbudowac drzewo decyzyjne [można by jeszcze mieć prawdopodobieństwo stopu, i do funkcji kosztu dodać średnią czas do podjęcia decyzji]

pokazywać maksymalny prototyp

==> removed.tex <==
%The \textbf{original pruning} presented in~\cite{chen2019looks} finds the $\kappa$-nearest \jacek{jakioś dziwna ta litera?} training patches to each prototype $p$. If less than $\tau$ out of $\kappa$ patches come from the class of prototype $p$, then it is assumed that $p$ most likely corresponds to the background, and it is removed along with its last layer connections. Finally, ProtoPNet optimizes the last layer to boost accuracy. \todo{should we write here about 6 and 4?}

% \begin{algorithm}[t]
% \SetAlgoLined
% \textbf{Input:} set of all prototypes $P=\{p_i\}_i$; weight of fully connected layer $w_h$; percentage of prototypes to merge per step $\zeta$\\
% \For {$(p, \tilde{p}) \in P^2$ {\normalfont among } $\zeta$ {\normalfont percent of the most similar pairs of prototypes}} {
%     assign $\tilde{p}$ to classes to which $p$ is assigned (other assignments of $\tilde{p}$ remain unchanged)\\
%     $w_h(\tilde{p}) \xleftarrow{} w_h(\tilde{p}) + w_h(p)$\\
%     remove prototype $p$ and its weights $w_h(p)$
% }
% \KwResult{updated $\{p_i\}_i$ and $w_h$}
% \caption{One step of merge-pruning}
% \label{alg:pruning}
% \end{algorithm}

% Additionally, we plot the KDE of the normalized distance between prototypes in Figure~\ref{fig:hist} and observe that for the data-dependent similarity metric there are more prototypes that are close to each other than for the $L_2$ metric which is uniformly spreading the smallest distance values. This leads us to an assumption that activation similarity is not only catching the similarity on the pixel level but also finds similar concepts on which the neural network is making a decision. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/hists.png}
%     \caption{Distributions of normalized distances between pairs of prototypes from ProtoPShare and a data-independent alternative. We observe the peak at the beginning of the former, resulting from finding similar concepts even for prototypes distanced according to Euclidean norm (like in the pair from Figure~\ref{fig:dd_di_similarity}). Notice that the initial parts of distributions are zoomed.}
%     \label{fig:hist}
% \end{figure}

% Results of the user study, shown in Figure~\ref{fig:user_study}, point out that the activation similarity between prototypes is better in merging the prototypes that share the same semantic meaning. Additionally, we made the Wilcoxon Signed-Rank test\footnote{The Wilcoxon signed test is designed to test a hypothesis about the location median of population distribution. We assume that the null hypothesis is a median of 0.75 whereas an alternative hypothesis we take that the median of user voices is less than 0.75. The voices for 'data-independent' we defined as -1, impossible to decide as 0, and ProtoPShare as 1.} (it may be used when the dependent variable is not normally distributed, what we have for the received data), which confirmed the effectivity of our method. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/user_study.png}
%     \caption{The results of the user study show the activation similarity between prototypes has better interpretability aspects.}
%     \label{fig:user_study}
% \end{figure}

% \subsection{Time of pruning}

% The process of pruning is quite straightforward. The fastest pruning will be the data-independent one as it does not need to push through the model all of the training images. However, the original and data-dependent pruning methods are similar in time requirements. The main bottleneck in the time needed to obtain the most effective model is the last layer optimization. 
% Additionally, we have implemented an efficient way of calculating the distances between prototypes which is shown in the supplementary material in the PyTorch framework. 

%\subsection{Prototypes of species of the same type}
%\todo{How does prototypes inside the type are shared between its species}

% \begin{table}
% \tiny
% \begin{center}
% \begin{tabular}{|l| c | c | c | c | c |c |}
% \hline
% \multirow{2}{*}{Model} & \multirow{2}{*}{No of prototypes} & \multicolumn{3}{|c|}{Optimized} & \multirow{2}{*}{Merging} & \multirow{2}{*}{Accuracy} \\
% \cline{3-5}
%  &  & Features & Prototype layer & Last layer &  &  \\
% \hline\hline
% \multirow{5}{*}{ResNet152} & \multirow{5}{*}{~1000} & No & No & Yes & Yes & $\mathbf{0.7361}$ \\
%  &  & No & Yes & Yes  & Yes & $0.7161$ \\
%  &  & Yes & Yes & Yes & Yes & $0.6821$ \\
%  \cline{3-5}
%  &  & \multicolumn{3}{c|}{5 prototypes per class} & No & $0.7151$ \\
%  \cline{3-5}
%  &  & \multicolumn{3}{c|}{joint learning} & No & $0.6938$ \\
% \hline\hline
% \multirow{5}{*}{ResNet34} & \multirow{5}{*}{400} & No & No & Yes  & Yes & $\mathbf{0.7472}$ \\
%   &   & No & Yes & Yes  & Yes & $0.6591$ \\
%   &   & Yes & Yes & Yes  & Yes & $0.6355$ \\
%   \cline{3-5}
%   &   & \multicolumn{3}{c|}{2 prototypes per class} & No & $0.7259$ \\
%   \cline{3-5}
%   &   & \multicolumn{3}{c|}{joint learning} & No  & $0.6833$ \\
% \hline\hline
% \multirow{5}{*}{DenseNet161} & \multirow{5}{*}{600} & No & No & Yes  & Yes & $\mathbf{0.7645}$ \\
%  & & No & Yes & Yes  & Yes & $0.7047$ \\
%  & & Yes & Yes & Yes  & Yes & $0.6526$ \\
%  \cline{3-5}
%  & & \multicolumn{3}{c|}{3 prototypes per class} & No & $0.7075$ \\
%  \cline{3-5}
%  & & \multicolumn{3}{c|}{joint learning} & No & $0.6823$ \\
% \hline\hline
% \multirow{5}{*}{DenseNet121} & \multirow{5}{*}{1000} & No & No & Yes  & Yes & $\mathbf{0.7472}$ \\
%  & & No & Yes & Yes  & Yes & $0.6836$ \\
%  & & Yes & Yes & Yes  & Yes & $0.6612$ \\
%  \cline{3-5}
%  & & \multicolumn{3}{c|}{5 prototypes per class} & No & $0.4621$ \\
%  \cline{3-5}
%  & & \multicolumn{3}{c|}{joint learning} & No & $0.3764$ \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Different learning strategies for smaller number of prototypes.}
% \label{tab:diff_optims}
% \end{table}

% \todo{}
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.88\textwidth]{figures/Removed but should not be (3).pdf}
%     \caption{Sampled non-background prototypes removed from DenseNet161 after applying original prototype pruning from~\cite{chen2019looks}. One can observe that the original pruning removes many meaningful prototypes which are shared between the classes.}
%     \label{fig:aaa}
% \end{figure*}

% \begin{figure*}
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \end{center}
%   \caption{Example of a short caption, which should be centered.}
% \label{fig:short}
% \end{figure*}

% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline
% Method & Frobnability \\
% \hline\hline
% Theirs & Frumpy \\
% Yours & Frobbly \\
% Ours & Makes one's heart Frob\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Results.   Ours is better.}
% \end{table}

